Near to Mid-term Risks and Opportunities of Open-Source Generative AI

In the next few years, applications of Generative AI are expected to revolutionize a number of different areas, ranging from science & medicine to education. The potential for these seismic changes has triggered a lively debate about potential risks and resulted in calls for tighter regulation, in particular from some of the major tech companies who are leading in AI development. This regulation is likely to put at risk the budding field of open-source Generative AI. We argue for the responsible open sourcing of generative AI models in the near and medium term. To set the stage, we first introduce an AI openness taxonomy system and apply it to 40 current large language models. We then outline differential benefits and risks of open versus closed source AI and present potential risk mitigation, ranging from best practices to calls for technical and scientific contributions. We hope that this report will add a much needed missing voice to the current public discourse on near to mid-term AI safety and other societal impact.

==> sections/2_def_and_taxonomy/tables/classification_sample.tex <==

\begin{table*}
    {
    \scriptsize
    \begin{tabular}{
        >{\hspace{0em}}m{0.06\linewidth}|
        >{\centering\hspace{0em}}m{0.04\linewidth}>{\centering\hspace{0em}}m{0.04\linewidth}>{\centering\hspace{0em}}m{0.04\linewidth}|
        >{\centering\hspace{0em}}m{0.04\linewidth}>{\centering\hspace{0em}}m{0.05\linewidth}>{\centering\hspace{0em}}m{0.04\linewidth}|
        >{\centering\hspace{0em}}m{0.05\linewidth}>{\centering\hspace{0em}}m{0.07\linewidth}|
        >{\centering\hspace{0em}}m{0.05\linewidth}>{\centering\hspace{0em}}m{0.05\linewidth}|
        >{\centering\hspace{0em}}m{0.06\linewidth}|>{\centering\arraybackslash\hspace{0em}}m{0.08\linewidth}
    }
    
    \toprule
    \multirow{3}[6]{0.06\linewidth}{\hspace{0em}\textbf{Model}} & \multicolumn{6}{c}{\textbf{(1) Training}} & \multicolumn{4}{c}{\textbf{(2) Evaluation}}                                                                      & \multicolumn{2}{c}{\textbf{(3) Deployment}}  \\ \cmidrule{2-13}
    
    & \multicolumn{3}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Data}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{2}{c}{\textbf{Data}} & \textbf{Code}          & \textbf{Data}                                                                \\ \cmidrule{2-13} 
    
    & \textbf{Pre-Training}  & \textbf{Fine-tuning}   & \textbf{Alignment} & \textbf{Pre-Training}                         & \textbf{Supervised FT} & \textbf{Alignment} & \textbf{General Eval}  & \textbf{Automatic Safety Eval}         & \textbf{Utility Benchmarks} & \textbf{Safety Eval Datasets}   & \textbf{Inference}     & \textbf{Model Architecture and Weights} \\
    \midrulenospacing
    
    \multicolumn{13}{c}{$\dots$} \\ \hline
    
    OpenLLaMA                                                 & \CFiveTable\par{}(Apache 2.0)   & \NATable                 & \NATable                          & \DFourTable\par{}(RedPajama Data)                      & \NATable                          & \NATable                          & \CFiveTable\par{}(Apache 2.0)         & \NATable                                       & \NATable                               & \NATable                                & \CFiveTable\par{}(Apache 2.0)   & \DFiveTable\par{}(Apache 2.0)                                                         \\\hline
    \multicolumn{13}{c}{$\dots$} \\ \hline

    Falcon                                                    & \COneTable                   & \COneTable                   & \COneTable                            & \DFourTable\par{}(ODC-By)                              & \DOneTable                             & \DOneTable                             & \COneTable                         & \NATable                                       & \NATable                               & \NATable                                & \CFiveTable\par{}(Apache 2.0)   & \DFiveTable\par{}(Falcon-180B Data)                                                   \\\hline

    \multicolumn{13}{c}{$\dots$} \\ \hline

    Gemini                                                    & \COneTable                   & \COneTable                   & \COneTable                            & \DOneTable                                           & \DOneTable                             & \DOneTable                             & \COneTable                         & \COneTable                                         & \COneTable                                 & \COneTable                                  & \COneTable                   & \DTwoTable 
    \\\bottomrulenospacing
    \end{tabular}
    }
    \caption{\textbf{Model Pipeline Classification} (full table in Appendix \ref{app:taxonomy_tables}, Table \ref{tab:classification_full}): openness classification of components of the training, evaluation and deployment pipelines of currently available large language models. “N/A” in this table corresponds to "Not Applicable”, whereas “?” means the information is not publicly available. If a model has more than one source of code or data source for a given component, the final classification is taken by considering the strictest license. For conciseness, in the table header we use "FT" as a stand in for "Fine-Tuning".}
    \label{tab:classification_sample}
\end{table*}

==> sections/2_def_and_taxonomy/tables/licenses_table_sample.tex <==
\begin{table*}[t]
    \begin{adjustwidth}{0pt}{0pt}
    {
    \scriptsize
    \centering
    \begin{tabular}{>{\hspace{0pt}}m{0.10\linewidth}>{\centering\hspace{0pt}}m{0.07\linewidth}>{\centering\hspace{0pt}}m{0.09\linewidth}>{\centering\hspace{0pt}}m{0.09\linewidth}>{\centering\hspace{0pt}}m{0.09\linewidth}>{\centering\hspace{0pt}}m{0.09\linewidth}>{\centering\hspace{0pt}}m{0.11\linewidth}>{\centering\hspace{0pt}}m{0.07\linewidth}>{\centering\arraybackslash\hspace{0pt}}m{0.07\linewidth}}
    \toprule
    \textbf{License}        & \textbf{Research} & \textbf{Commercial Purposes} & \textbf{Modify as Desired} & \textbf{Copyright derivative work} & \textbf{Other license for derivative} & \textbf{Final score}            & \textbf{Code Openness} & \textbf{Data Openness}  \\ \midrulenospacing
    MIT/Mod. MIT            & Y                 & Y                            & Y                          & Y                                  & Y                                     & 5\par{}(Restriction free)       & \CFiveTable                     & \DFiveTable                      \\ \hline
                  &                  &                             & $\dots$                          &                                   &                                      &        &                      &                       \\ \hline
    Falcon-180B Data        & Y                 & Y                            & Y                          & Y                                  & Y                                     & 5\par{}(Restriction free)       & \NATable                    & \DFiveTable               \\ \bottomrulenospacing
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{\textbf{License Openness Taxonomy} (full table in Appendix \ref{app:taxonomy_tables}, Table \ref{tab:licenses_full}): categorization of commonly used licenses in a variety of relevant open source criteria, and resulting code and data openness categories.}
    \label{tab:licenses_small}
    \end{adjustwidth}
\end{table*}


==> sections/2_def_and_taxonomy/tables/model_list_sample.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}
    {
    \scriptsize
    \centering

    \begin{tabular}{>{\hspace{0pt}}m{0.11\linewidth}>{\centering\hspace{0pt}}m{0.12\linewidth}>{\centering\hspace{0pt}}m{0.08\linewidth}>{\centering\hspace{0pt}}m{0.09\linewidth}>{\centering\hspace{0pt}}m{0.12\linewidth}>{\centering\hspace{0pt}}m{0.13\linewidth}>{\centering\hspace{0pt}}m{0.15\linewidth}>{\hspace{0pt}}m{0.00001\linewidth}}

    \toprule
    \multirow{2}[6]{\linewidth}{\hspace{0pt}\textbf{Model}} & \multirow{2}[6]{\linewidth}{\hspace{0pt}\Centering{}\textbf{Developer}} & \multirow{2}[6]{\linewidth}{\hspace{0pt}\Centering{}\textbf{Largest Model Size (params)}} & \multirow{2}[6]{\linewidth}{\hspace{0pt}\Centering{}\textbf{Release Date}} & \multicolumn{3}{>{\Centering\hspace{0pt}}m{0.41\linewidth}}{\textbf{Impact Metrics}} & \\ \cmidrule{5-7}
    
    & & & & \textbf{ChatBot Arena Elo Rating} & \textbf{Google Scholar Citations} & \textbf{HuggingFace Downloads Last Month} & \\ \midrulenospacing
    \multicolumn{8}{c}{$\dots$} \\ \hline
    OpenLLaMA                                                 & \DevNonProfit{UC Berkeley}                                                               & 13B                                                                                        & 06/2023                                                                      & N/A                               & N/A                               & 58,991                                    & \\ \hline
    \multicolumn{8}{c}{$\dots$} \\ \hline
    Falcon                                                    & \DevGovernment{TII}                                                                       & 180B                                                                                       & 09/2023                                                                      & 1,035                             & 65                                & 1,341,297                                 & \\ \hline
    \multicolumn{8}{c}{$\dots$} \\ \hline
    Gemini                                                    & \DevCompany{Google DeepMind}                                                           & N/A                                                                                        & 12/2023                                                                      & 1,111                             & N/A                               & N/A                                       &
   \\ \bottomrulenospacing
    
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{\textbf{Model Information} (full table in Appendix \ref{app:taxonomy_tables}, Table \ref{tab:model_list_full}): table containing the basic information about each of the models classified under the openness taxonomy. Developers highlighted in \colorbox{CompanyColor}{purple} correspond to companies, in \colorbox{NonProfitColor}{pink} are non-profit entities, and in \colorbox{GovernmentColor}{light blue} are government institutes. All data accessed on 28th of December 2023.}
    \label{tab:model_list_small}
\end{table*}

==> sections/3_regulatory/3_regulatory.tex <==
\section{Regulatory Landscape, Governance and Geopolitics}
\label{sec:regulation}

\subsection{The US Regulatory Landscape}
On October 30, 2023 US President Biden signed an executive  order (EO) on the Safe, Secure, and Trustworthy Development and Use of Artificial Intelligence~\citep{house_fact_2023}. The order is generally considered to represent a wide range of interests. There has been some criticism, however, about the influence of a handful of tech billionaires, with Politico detailing the extent to which certain parties were confirmed to be present at closed meetings~\citep{bordelon_think_2023}. This criticism follows on previous concern that the Congressional hearings were unduly influenced by industry given both the nature of certain remarks as well as closed events like a private dinner that was not open to review or feedback. 

On the one hand, the US Regulatory landscape evinces a holistic view that accounts for a variety of interested parties and tries to achieve a balance between regulation and innovation through responsible innovation. On the other hand, the US regulatory landscape cannot be seen as divorced from the larger lobbying forces under which some groups, including the leading industry players, may hold outsized influence. As Harvard scholars Schneider and Sanders write, the Biden act represents ``a contest about control and power, about how resources should be distributed and who should be held accountable''~\citep{noauthor_think_nodate}. Brendan Bordelon of Politico goes on to suggest that the act ``papers over'' the ``growing tension between Washington’s rival AI factions''~\citep{schneier_opinion_2023}. 

Schneider and Sanders categorize the different factions represented in the executive act as  ``\textit{doomsayers,}'' ``\textit{reformers}'' and ``\textit{warriors.}'' Doomsayers highlight the existential risk AI poses. Reformers focus on the already extant series of harms being perpetrated, as well as potential looming economic disruption. Warriors are concerned with the geopolitical sphere amid worries the US will lose its global dominance. Each of these groups highlights the risks and benefits according to their particular concerns and viewpoints. The doomsayers have come under the most criticism for overstating the extent to which fears of existential risk are a dominant viewpoint among AI researchers and developers~\citep{noauthor_how_nodate}. Adding to this concern is the fact that highlighting existential risk may benefit leading industry players, for whom regulation could help as an insincere stratagem to cement their market advantage by handicapping smaller competitors.

Reflecting these various positions, the EOpresidential act outlines the various risks of AI and calls for various government agencies to develop plans that include developing critical infrastructure for defense and governmental support of AI research. NIST is tasked with developing practices surrounding their AI Risk Management Framework. To this end, NIST is in the process of creating the US AI Safety Institute Consortium to include members from state and local governments, universities, non-profits, and industry. 

The Biden and Harris Executive Order stands apart from the EU regulatory landscape in one key aspect: models with ``\textit{freely available weights.}'' In the EU, Models below a specific compute budget threshold have been protected from regulation, at least for the present. This is seen as either a positive protection of competition and development or an unfortunate capitulation to lobbying depending on the perspective. The Biden act, on the other hand, specifically calls out open-source models as a locus of potential risk. 

\subsection{Regulation in the EU: The EU AI Act}

The EU AI Act is widely regarded as the world’s first attempt at a comprehensive regulation of AI systems. It is important to recognise that this attempt did not happen in a vacuum, but followed and built upon other generalist regulatory initiatives, such as the General Data Protection Regulation (GDPR, 2016), and the Digital Markets Act (DMA, 2012). It is instructive to realise that the EU started examining the compatibility of the GDPR and AI as early as in 2020~\citep{european_parliament_directorate_general_for_parliamentary_research_services_impact_2020}. Understanding the Act’s future influence on open-source foundation models does necessitate a holistic investigation. 

On December 9th, 2023, the Act was provisionally agreed between the European Parliament and the European Council. During the 3-day round of negotiations, the Act’s scope was tightened. It was clarified that the Act does not apply outside of European law, does not infringe on the security competences of the member states or so-entrusted entities, nor any military or defence applications. Importantly, it was clarified that the Act would not apply to sole purposes of research and innovation, nor other non-professional use. The EU AI Act act aligns central AI taxonomies with those proposed by the OECD, defining an AI systems as ``\textit{a machine-based system that is designed to operate with varying levels of autonomy and that can, for explicit or implicit objectives, generate outputs such as predictions, recommendations, or decisions that influence physical or virtual environments.}''~\citep{AIACT_announcement}. 

\paragraph{Roles.} The Act distinguishes between the roles of provider, deployer, importer and distributor, and a distinction is made between models provided or deployed from within the EU, or from the outside in a third-country. Providers, i.e. those that develop AI systems with the intention to bring them to the market, whether paid or free, have pre-market obligations including an initial risk assessment, risk-specific compliance, as well as risk-specific post-market obligations. Deployers are users of AI systems that don’t fall within a small number of non-professional use cases.

\paragraph{Risk classification systems.} The EU AI Act defines two parallel risk classification systems for the regulation of AI models: one for general-purpose AI (GPAI) models and foundation models, and one for AI models of specific purpose. Models of specific-purpose are regulated according to a tiered risk system based on use cases, ranging from prohibited systems, high risk systems, to minimal risk systems. Prohibited systems are those with unacceptable risk to people’s safety, security, and human rights. According to Article 28(2a), providers of high risk systems are subject to compliance obligations, including the establishment of risk and quality management systems, data governance, human oversight, cybersecurity measures, postmarket monitoring, and maintenance of the required technical documentation~\citep{ai_act_compliance_checker}. It is to be expected that these obligations will be further detailed in later, sector-specific regulation. Providers of minimal risk systems may attract limited obligations if interacting directly with people or if they manipulate or generate visual or audio content, but otherwise are only subject to limited transparency requirements.

\paragraph{General-purpose AI model.} According to the December 6th Compromise Proposal~\citep{noauthor_preparing_nodate}, ‘General-purpose AI model’ means an AI model, including when trained with a large amount of data using self-supervision at scale, that displays significant generality and is capable to competently perform a wide range of distinct tasks regardless of the way the model is released on the market and that can be integrated into a variety of downstream systems or applications
The EU AI Act imposes particular regulation on providers of general-purpose AI models of ``\textit{systemic risk}'' (Article D), which it defines to be all models for which ``the cumulative amount of compute used for its training measured in floating point operations (FLOPs) is greater than $10^{25}$''. Such providers need to register their model with the European Commission, and need to ensure a wide-ranging catalogue of safety and security criteria. The EU AI Act does appear to leave provisions for adjusting various technical criteria related to ``\textit{systemic risk}'' classifications in the future~\citep{benedict_openness_2023}.  


\paragraph{Exemptions for providers of open source AI systems}
The latest publicly known draft of the EU AI Act, Commission Compromise Proposal v2, as leaked by Politico~\citep{AIAct}, contains wide-ranging exemptions for providers of certain AI systems provided under free and open source software licences. To be exempt, the models provided may not fall within the ``\textit{systemic risk}'' category, or otherwise exhibits harmful behaviour of unacceptable risk, such as manipulative or exploitative behaviour, social scoring purposes, and certain biometric identification (Title II), or certain AI systems that leave the user uninformed about their interaction with an AI system, emotion recognition systems or biometric categorisation systems, or AI systems producing ``\textit{deep fakes}'' (Title IV Article 52~\citep{AIACT_announcement}). 

\paragraph{Are ``\textit{open models'' synonymous to ``open source models}''?}
Interestingly, the leaked draft~\citep{AIAct} distinguishes the above from providers of ``\textit{pre-trained AI models that are made accessible to the public under a licence that allows for the access, usage, modification, and distribution of the model, and whose parameters, including the weights, the information on the model architecture, and the information on model usage, are made publicly available,}''. It is to be noted that the term ``\textit{open source model}'' is not used explicitly and the degree of legal overlap with open source software is not immediately clear, and hence we will refer to such models as ``\textit{open models}''. Open models are not exempt from Article C(1)[(c),(d)], as well as Article D and Article 28(2a), the latter governing third-party obligations ``along the AI value chain of providers, distributors, importers, deployers or other third parties''~\citep{european_parliament_directorate_general_for_parliamentary_research_services_impact_2020} for high risk AI systems. 

\paragraph{Are open GPAI models subject to high risk obligations?}
It is here that the EU AI Act becomes slightly confusing. On the one hand, GPAI models attract their very own risk categorisation into ``basic'', and ``systemic'' risk. On the other hand,~\citet{AIAct} seemingly reimposes ``\textit{high risk}'' regulation onto GPAI models if they are open. If Article 28(2a) is indeed meant to apply to open GPAI models, then, in our assessment, this may pose the perhaps biggest legal onus on providers of open GPAI models, insofar as GPAI models, by definition, might be readily used, and trivially adapted, for a wide range of tasks, including those in high risk categories, such as law enforcement, career-critical educational or vocational contexts, or credit scoring. Specifically, Article 28(2a) demands that ``\textit{The provider of a high risk AI system and the third party that supplies tools, services, components or processes that are used or integrated in the high risk AI system shall, by written agreement specify the information, capabilities, technical access, and or other assistance, based on the generally acknowledged state of the art, that the third party is required to provide in order to enable the provider of the high risk AI system to fully comply with the obligations under this Regulation.}'' It remains unclear to what extent providers of open GPAI models could fulfil obligations under Article 28(2a) by explicitly prohibiting high risk downstream use in their model licences. 

\paragraph{Transparency requirements.}
Under any circumstances, providers of open GPAI models are responsible for transparency obligations according to Article C(1)[(c),(d)]. These transparency requirements include respecting existing Union copyright law  (Article C(1)[(c)]) according to Article 4(3) of the (Digital Single Market) Directive (EU) 2019/790 [14], and the need to make a ``\textit{sufficiently detailed summary of the content used for training of the general-purpose AI model}'' (Article C(1)[(d)]). The consequences of these transparency requirements for open GPAI model providers have been examined in~\citep{benedict_openness_2023}. Importantly, Directive (EU) 2019/790 expands GDPR regulation to copyright owners who share content online, meaning that key GDPR rights, such as the ``\textit{right to opt out}'' (Article 7 GDPR) [15] would require that copyright owners could ask for their data to be removed from open GPAI model training data. Another interesting aspect is the question of what constitutes a ``sufficiently detailed summary'' of training data~\citep{benedict_openness_2023}.

\paragraph{Are providers of open models obliged to implement watermarking provisions?}
Interestingly, the Politico leak~\citep{AIAct} shows traces of what may have been last-minute changes to watermarking obligations for GPAI, and hence open GPAI, model providers. Specifically, in Article C(1)[(e)] on watermarking provisions one finds a remark that watermarking provisions have been moved to Title IV Article 52 instead. The now deleted Article C(4) would have explicitly made open GPAI models subject to watermarking provisions.

\paragraph{Draft Forensics.}
Reading the Commission Compromise v2 closely~\citep{AIAct}, we identify several confusing and seemingly contradicting statements. For example, \citet{AIACT_announcement} introduces Article D(4), which states that Article C(4) exemptions for open GPAI models do not apply to GPAI models of systemic risk. However, the preamble states that Article C(4) was bracketed (which it is not) and would be deleted. In addition, we note that Article 28(2a) obligations to open models are bracketed in the preamble without further comment~\citep{AIACT_announcement}. This may indicate ongoing debate over whether high risk obligations should indeed apply to providers of open models, including open GPAI models. We cannot help but note that these inconsistencies seem, in fact, not merely clerical, but may indeed reflect a high-level confusion over the very core of the EU AI Act: namely the seemingly conflicting risk categorisations of GPAI models versus non-GPAI models, made blatantly visible in the nexus of open GPAI model regulation. 

\paragraph{Measures in support of innovation and small companies.}
In apparent response to criticism concerning the innovation-friendliness of prior comprehensive EU legislation, such as the GDPR, Commission Compromise v1 introduced several measures in support of innovation, such as e.g. allowing for regulatory sandboxes that provide controlled environments for developing, testing, and validating innovative AI systems to be used for real world tests under suitable conditions. In addition, a number of additional actions are announced that are meant to exempt smaller companies from certain regulation. We find it conceivable that such measures could, in principle, amplify the effect of open GPAI models on innovation in the startup scene.

\paragraph{Obligations for providers of open models in third countries.}
The EU AI Act applies to both providers and deployers located in a third country where the output produced by the system is used in the EU~\citep{european_parliament_directorate_general_for_parliamentary_research_services_impact_2020}. Third-country providers of open GPAI models aiming at the EU market therefore will need to fulfill the obligations discussed in this government. While it currently seems unclear how third country providers would choose to fulfill potential obligations surrounding high risk or systemic risk efficiently, it seems that underlying obligations stemming from DSM and GDPR regulation could be fulfilled through existing routes, such as \href{https://www.dataprivacyframework.gov/s/}{transatlantic data sharing agreements}.


\paragraph{Going forward.}
At the time of writing (January 2024), the EU AI Act is still in the recital phase~\citep{noauthor_recitals_nodate}, meaning that further changes to the Act are not expected until it is submitted for ratification by the Committee of Permanent Representatives (Coreper) in, supposedly~\citep{mukherjee_explainer_2023}, early 2024. At the Coreper, a blocking minority of as few as four countries could theoretically derail the law ahead of its publication in the official journal. While Germany, Italy, and France conceded their various calls for exemptions in December, Emmanuel Macron has since been vocal on his stance that the EU AI Act may still hamper innovation~\citep{abboud_eus_2023}. 

As to whether the seeming confusion of to what extent non-GPAI risk obligations should apply to open GPAI models will significantly impact the providers of open GPAI models will also be affected by whether usage restrictions and the availability of suitable harmonised standards (see bracketed Article C(3)) will allow providers of open GPAI models to escape from the regulatory maze. As such, with respect to open models, the EU AI Act could still result in workable practices but fail to provide a plausible high-level categorisation of AI risks.




\subsection{The Middle East}


\textbf{Saudi Arabia } In response to Saudi Arabia's newly announced 2030 Vision, which was introduced by the Crown Prince Mohammed Bin Salman in April 2016, numerous government entities have emerged where advanced technology is their main focus. A key development is the August 2019 establishment of the Saudi Data and AI Authority (SDAIA) by a royal decree to facilitate advancing the 2030 vision with a National Center for AI as one of its arms. Saudi Arabia, through SDAIA, has adapted and released its first version of AI ethics in September 2023 \cite{SDAIA_AI_ethics}. The document outlines Saudi's stance on AI risks, categorized from minimal to unacceptable risks with a comprehensive risk management plan covering data, algorithms, compliance, operations, legality, and regulatory risks. The AI ethics strongly supports the transparent development and deployment of AI. The AI ethics reads ``Transparent and explainable algorithms ensure that stakeholders affected by AI systems... are fully informed when an outcome is processed by the AI”. Moreover, SDAIA has quickly embraced the generative AI wave. In collaboration with NVIDIA, SDAIA developed ``Allam" \cite{Allam}, Saudi Arabia's first national-level LLM model, an Arabic LLM designed to provide summaries and answer questions, drawing information from cross-checked online sources. While Allam was closed source %[\textcolor{red}{use here the categorization and taxonomy used in our report}] 
 and only a beta version interface is accessible, there are still several pieces of evidences that Saudi Arabia is in favor of open-source. For instance, the Digital Government Authority \cite{digital_gov_auth} issued free and open-source government software licenses to 6 government agencies in 2022. This entails reviewing and publishing the source codes "in a way that opens the field of cooperation and unified standards among government agencies". The general directions with the laid down ahead-of-its-time thorough compliance regulations, stated principles, and open-source government suggests that Saudi Arabia is in the direction of supporting open-source.



\textbf{United Arab Emirates } In October 2017, the UAE Government launched the pioneering ``UAE Artificial Intelligence Strategy'' \cite{UAE_strategy_Gov}, spanning sectors from education to space. Shortly after, Omar Al Olama became the world's first AI minister. Studies \cite{talib2017open} highlight significant awareness of open-source software in the UAE. This all indicates that similarly to Saudi Arabia, the UAE has had the ground fertile for slowly adopting open-source policies. Following the UAE AI strategy, the UAE has been in favor of open-source in their policies, for instance, as stated in the strategy ``Objective 7: Provide the data and the supporting infrastructure essential to become a test bed for AI" and that ``The UAE has an opportunity to become a leader in available open data for training and developing AI systems". Moreover, the strategy states that ``The UAE’s ambition is to create a data-sharing program, providing shared open and standardized AI-ready data, collected through a consistent data standard". 

%If implemented this will place UAE in terms of our proposed taxonomy on the \textcolor{red}{C3 to C4 level}. More recently, the UAE, notably through the Technology Innovation Institute (TII), has recently open-sourced Falcon \textcolor{red}{cite falcon}, including its remarkable 180B parameter model trained on 3.5 trillion tokens. This model, launched ahead of hugging face's pre-trained models, is now available as an open-source LLM for both research and commercial purposes, reflecting the UAE's proactive stance on open-sourcing.

% \paragraph{Summary.}
% Both Saudi Arabia and the United Arab Emirates (UAE) exhibit a positive attitude towards open source initiatives, particularly in the realm of artificial intelligence (AI). Saudi Arabia, through its governmental bodies like the Saudi Data and AI Authority (SDAIA), emphasizes transparency and accountability in AI development, with a focus on open-sourcing government software licenses. Similarly, the UAE, under its Artificial Intelligence Strategy, aims to become a leader in open data for AI development, evidenced by initiatives like the open-sourcing of Falcon, a large language model, by the Technology Innovation Institute (TII). Both nations recognize the importance of open source in fostering innovation and collaboration within their burgeoning AI ecosystems.




\subsection{Other countries}

Besides the countries addressed above, at least 35 ~\citep{noauthor_oecds_nodate} other countries have deployed some form of AI policy or regulation~\citep{australian_2024}. Nonetheless, by January 2024, none of those have issued policies specifically about open AI, suggesting the leading geopolitics of regulation lies on the aforementioned forums, mainly the EU and the US.
 
\footnote{Argentina, Australia, Canada, Chile, Colombia, Costa Rica, Egypt, Iceland, India, Israel, Japan, Kazakhstan, Kenya, Korea, Mauritius, Mexico, Morocco, New Zealand, Nigeria, Norway, Peru, Rwanda, Serbia, Singapore, South Africa, Switzerland, Thailand, Tunisia, Turkey, Uganda, Ukraine, Uruguay, Uzbekistan, and Vietnam.}
 
It is important to acknowledge that some countries have issued policies specifically on Generative AI, addressing mainly sector-based issues. This is the case for example of Australia (i.e. guidelines for schools~\citep{noauthor_interim_nodate,} and for the public sector~\citep{noauthor_guidelines_nodate}), Canada (i.e. general guidelines link and general principles~\citep{noauthor_guidelines_nodate,}], New Zealand (i.e. judicial system, ~\citep{kaldestad_new_2023}], Norway (i.e. consumer protection, link), and Singapore (i.e. financial sector, ~\citep{noauthor_mas_nodate}, and sandboxes, ~\citep{noauthor_first_nodate}). We can also point that other few countries are in the process of running public consultations on how to regulate generative AI, such as the case of Chile~\citep{httpsmagnetcl_articulo_nodate} and Uruguay~\citep{noauthor_mesa_nodate}.
 
It is also relevant to point out that AI policies started to appear mainly from 2017 onwards~\citep{noauthor_pl_nodate-1}, while generative AI and open AI attracted attention of policymakers from mid-2023 onwards. As a hypothesis, we can suggest that even countries that had advanced AI regulatory debates for many years have not reached the point to debate generative AI, and even less, open AI. Brazil is a good case to illustrate that.  
 
Brazil is working on two main legislative proposals to regulate AI, one inspired in the US framework (Bill no. 21, from 2021) and another inspired on the EU framework (Bill No. 2338, from 2023). None of those have so far provision on generative AI or open AI. The EU-inspired bill is of particular interest. This proposal has been heavily influenced by the EU AI Act debate. Although heavily altered to address local demands, and enhanced with a human-rights approach that goes even beyond the EU framework~\citep{noauthor_road_nodate}, no congressional debate addressed the issues of generative AI or open AI by the end of 2023. In fact, the only policy window in the country, so far, is a public consultation opened by the Supreme Electoral Count on AI-generated electoral materials~\citep{noauthor_eleicoes_nodate}.


\subsection{Geopolitics.}


On the global stage, the Bletchley Declaration \href{https://www.gov.uk/government/publications/ai-safety-summit-2023-the-bletchley-declaration/the-bletchley-declaration-by-countries-attending-the-ai-safety-summit-1-2-november-2023}{[link]} and the G7 Hiroshima AI Process \href{https://www.mofa.go.jp/files/100573466.pdf}{[link]} are pioneering efforts to establish standards and guiding rules for AI developers and users. These initiatives aim to engage emerging national AI safety organizations around the world to form a network aligned with shared agreements and policies, which will influence ongoing discussions about open-source AI. 

The EU is advocating for regulation with its proposed EU AI Act, which awaits approval from individual EU countries but is already influencing AI regulatory standards. 

With the rise of AI technologies, nations are entering a new kind of arms race. Leading countries have the opportunity to use AI as a means of soft power—even as an open-source tool—by providing, maintaining, and updating AI systems for developing nations, thus gaining strategic influence over AI implementation in those countries. 



==> sections/5_medium_term/5_medium_term.tex <==
\section{(Old) Medium-term Impact of Open Source Models}

% {\color{red} Merge this section with the near term}

% \textcolor{red}{TODO: Section introduction}

% \paragraph{Economic impacts}
% Open-source/closed-source effects both on the general economy and also on the GenAI market

% {\color{red}
% (Merged with the near-term point on economic impact
% \paragraph{Generative AI Powered Agents and Integration within Other Systems}

% The widespread adoption of generative AI systems has so far mostly been limited to either text or images, or a combination of the two modalities. While these have been shown to be useful due to their standalone capabilities, there is currently an ambitious drive towards extending and integrating them in broader, agent-based frameworks where the output includes the performance of actions (\href{https://www.adept.ai/blog/act-1}{Adept’s blog post}, \href{https://press.aboutamazon.com/2023/7/aws-expands-amazon-bedrock-with-additional-foundation-models-new-model-provider-and-advanced-capability-to-help-customers-build-generative-ai-applications}{Amazon’s press release}).

% This expansion and integration of generative AI systems into agents is still at its infancy today (\href{https://arxiv.org/abs/2304.03442}{Park et al., 2023}), yet it is probable the technology has reached a high level of maturity within the mid-term horizon, with physical electronic devices incorporating this technology also becoming commonplace (\href{https://www.theverge.com/2023/11/9/23953901/humane-ai-pin-launch-date-price-openai}{AI Pin announced by Humane at CES 2024}).
% Both digital and physically embodied generative AI agents could possess the capability to interact and collaborate with other agents, thus enhancing their efficiency and effectiveness in accomplishing a variety of tasks.

% There are different levels of impacts associated with building and integrating these generative AI powered systems through closed and open source models.

% In the case of closed source models accessed via an API, the end product developers will be: (1) reliant on external providers for crucial capabilities of their product with potentially limited control and maintainability, (2) dependent on the continued availability of the required closed source model, and (3) unable to thoroughly audit the models and understand how their data is being used. In contrast, for open source models: (1) developers can update the model as they deem fit, (2) developers have complete clarity about the model in use and deploy it on-device, and (3) the end product developers control the data pipeline, significantly enhancing privacy and auditing capabilities (\href{https://sloanreview.mit.edu/article/use-open-source-for-safer-generative-ai-experiments/}{Culotta and Mattei, 2023}) \footnote{Note that the ability to fully audit open source models depends not only on the model weights, but also on the pipeline components released, such as training and fine-tuning data for example.}

% From the perspective of benefits of closed source for the developers of the end product, it is possible that: (1) cheaper and faster inference due to economy of scale, and (2) the foundational models are likely to be more highly performant on a range of tasks (as development is probably 12-18 months ahead of the open source ones) (\href{https://www.theinformation.com/articles/metas-free-ai-isnt-cheap-to-use-companies-say}{Palazzolo, 2023}, \href{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}{Beeching et al., 2023}), although the performance gap from (2) is likely to be reduced in the future (\href{https://assets.publishing.service.gov.uk/media/653932db80884d0013f71b15/generative-ai-safety-security-risks-2025-annex-b.pdf}{UK, GOV, 2023}).
% }

% \paragraph{Changes to our relationship with information}

% \paragraph{Changes to civil society}

% Generative AI can be used to audit public and private institutions (\href{https://www2.deloitte.com/us/en/blog/accounting-finance-blog/2023/generative-ai-auditing.html}{Bible, 2023}), improve social service delivery (\href{https://www.callhandling.co.uk/generative-ai-in-charity-and-healthcare-sectors-balancing-risks-and-rewards/}{Call Handling, 2023}), and, support  public discourse through fact checking and moderation (\href{https://eprints.whiterose.ac.uk/206287/}{Althabiti et al., 2023}, \href{https://www.wired.co.uk/article/fact-checkers-ai-chatgpt-misinformation}{Morrish, 2023}). However, AI also poses to civil society in terms of privacy and intellectual property (IP) (\href{https://www.ohchr.org/sites/default/files/documents/issues/business/b-tech/taxonomy-GenAI-Human-Rights-Harms.pdf}{UN B-Tech, 2023}, \href{https://cedpo.eu/wp-content/uploads/generative-ai-the-data-protection-implications-16-10-2023.pdf}{CEDPO AI Working Group, 2023}),  mis/disinformation that could be generated by these models (\href{https://www.sciencedirect.com/science/article/pii/S2405844024007588}{Raman et al., 2023}, \href{https://www.gov.uk/government/publications/frontier-ai-capabilities-and-risks-discussion-paper/safety-and-security-risks-of-generative-artificial-intelligence-to-2025-annex-b}{UK Gov, 2023}), bias, unfairness and discrimination (\href{https://www.ohchr.org/sites/default/files/documents/issues/business/b-tech/taxonomy-GenAI-Human-Rights-Harms.pdf}{UN B-Tech, 2023}, \href{https://www.gov.uk/government/publications/frontier-ai-capabilities-and-risks-discussion-paper/safety-and-security-risks-of-generative-artificial-intelligence-to-2025-annex-b}{UK Gov, 2023}, \href{https://www.bloomberg.com/graphics/2023-generative-ai-bias/}{Nicoletti et al., 2023}), among others.
% The success of such implementations and mitigations is, however, highly dependent on whether the available models are open or closed source.
% The use of GenAI systems by public institutions raises significant concerns due to the inability to independently audit these systems. This limitation fosters distrust, especially in their handling of bias, discrimination, and safety issues, as evidenced by past difficulties with closed source software audits (\href{https://committees.parliament.uk/work/1272/new-technologies-and-the-application-of-the-law/publications/}{UK Parliament}, \href{https://www.science.org/doi/10.1126/science.aax2342}{Obermeyer et al.}, \href{https://www.wired.com/story/opioid-drug-addiction-algorithm-chronic-pain/}{Szalavitz}).

% Open source models have made public a larger portion of their data pipelines, helping identify bias, IP violations, mis/disinformation and public trust issues earlier compared to closed ones. They also foster a culture of contributing and holding organizations accountable (\href{https://www.weforum.org/agenda/2021/07/civil-society-help-ai-benefits/}{Sanchez, 2021}). Government oversight might be permissible in closed source models (\href{https://www.instituteforgovernment.org.uk/explainer/artificial-intelligence-regulation}{Shepley and Gill, 2023}), but only open source models will allow for the aforementioned widespread community oversight.

% Generative AI models can also be used by adversarial actors. The control exerted by the developers of closed source systems may lower the probability of misuse but inadequate safety measures, cyberattacks or model leaks can also affect close-source models. This happened before with the original LLaMA which was originally released only for research purposes before being leaked online (\href{https://www.theverge.com/2023/3/8/23629362/meta-ai-language-model-llama-leak-online-misuse}{Vincent, 2023}).

% {\color{red}
% (Merged with the near-term point on research)
% \paragraph{Impact on research and independent auditing}

% Public institutions, particularly in AI research, depend on open-source software for its cost-effectiveness and transparency, driving innovation and rapid development. Restricting access to these resources can hinder progress. Public research, crucial for theoretical advances and independent audits, benefits greatly from sharing models and code. Additionally, open-source tools support diverse applications in various research fields, allowing for the development of tailored solutions efficiently.


% Auditing GenAI systems for safety and fairness by researchers, non-profit organisations, governments, journalists, and the general public is vital (\href{https://jamanetwork.com/journals/jamaophthalmology/article-abstract/2811505}{Taloni et al. 2023}, \href{https://www.bloomberg.com/graphics/2023-generative-ai-bias/}{Nicoletti at el}., \href{http://proceedings.mlr.press/v81/buolamwini18a/buolamwini18a.pdf}{Buolamwini and Gebru, 2018}, \href{https://www.pnas.org/doi/full/10.1073/pnas.1915768117}{Koenecke et al.}). Open-source models facilitate easier auditing than closed-source ones, which face issues like cost and data leakage. Some types of auditing might be only possible with techniques such as jailbreaking, might be prohibited by the service’s terms and conditions, or impossible to do in a black box fashion \citep{casper2024blackbox}.

% With open-source availability, research on GenAI can continue to evolve, positively impacting the trajectory of technological development (refer to figure). Open-source facilitates compliance with open research policies and supports 'AI for science' and 'AI for good' initiatives. Conversely, restricting open-source access would likely make GenAI technology less accessible to researchers, thereby diminishing its positive impact. Should open-source models be restricted, the most capable and impactful models might become unauditabe or underauditable, potentially leading to unchecked bias, fairness, and safety issues, disproportionately affecting underrepresented groups. Furthermore, the embedding of unauditable models in public systems could erode trust in these crucial institutions.
% }

\paragraph{Global disparities}

Generative AI (GenAI) is often celebrated as a global technology revolution, yet its adoption and impact exhibit stark global disparities. The design, implementation, and support of these models are tailored to a minority, despite GenAI being lauded as a technology for the whole world (\href{https://www.economist.com/leaders/2024/01/25/the-tantalising-promise-of-ai-for-the-emerging-world}{Economist}). It is important to acknowledge who is developing the  largest open source GenAI tools: for-profit companies largely headquartered in the West and Silicon Valley. The perspectives and values reflected in the open source models and choices that inform them are therefore linked to these actors.  

As aforementioned, current language models excel in few popular languages and regions but falter significantly for the majority of the world's languages. Centralized corporations generally lack the incentives to represent the world's linguistic and cultural diversity into a singular product, especially as this would result in worse performance and higher costs for their predominant markets. Even if feasible, ethical concerns arise over community rights in dictating their representation and management within these models. Conversely, open-source models offer adaptability and customization, allowing for the integration of local languages, cultures and knowledge. Examples of such adaptability are evident in BERT and LLAMA, which have dozens if not hundreds versions which have been finetuned by various communities to support new languages and cultural contexts.

The development and operation of commercial GenAI systems predominantly occurring in high-income countries leads to prohibitively high costs for low income countries. There's an inverse relationship between a language's global standing and the cost of implementing GenAI solutions for it (\href{https://arxiv.org/abs/2305.15425}{shameless plum}, \href{https://arxiv.org/abs/2305.13707}{Ahia et al.}).

The assumption that developers have the highest motivation to maintain safety and security standards does not always hold true for their users in lower-income countries (cite instances in Myanmar, Sri Lanka, and India with Facebook/WhatsApp). In fact, there is already evidence that the safety and security measures of popular commercial systems do not work if one uses them in a language other than English (cite).

Low- and middle-income countries are at risk of losing job sectors, such as call centres and software development, to automation by GenAI. These jobs, typically outsourced from high-income countries, may vanish without corresponding economic benefits. Furthermore, if the GenAI models do not work well in the local context or are not affordable, new jobs or economic improvements might not materialize. This automation could exacerbate economic disparities, with benefits accruing in high-income countries while low and middle-income countries face job losses without viable alternatives (\href{https://www.imf.org/en/Blogs/Articles/2024/01/14/ai-will-transform-the-global-economy-lets-make-sure-it-benefits-humanity}{Georgieva 2024}).

The absence of open-source models and the dominance of closed-source systems could limit opportunities for countries outside the primary markets for these systems. Such disparities can manifest in inadequate language support, limited culturally relevant content, higher costs, and less effective safety measures. The decisions made by distant commercial entities rarely align with local interests. At the same time, embracing open-source GenAI can dramatically alter this landscape. It empowers communities to develop models suited to their unique contexts and needs, fostering innovation and ensuring safety, security, and reduced bias in their local environments. Critically, open-source will also support innovation in these places which would not be possible with a closed-source system. This approach not only nurtures global innovation but also has the potential to bridge the widening inequality gap, offering a more equitable and inclusive future for GenAI.


% \paragraph{Data incest/exhaustion}

% Data exhaustion is emerging as a critical concern, especially as training on synthetic data quality and diversity gradually diminishes \citep{alemohammad2023self}. Closed GenAI systems present a mixed landscape. Pros include the likelihood of for-profit organizations investing in maintaining the integrity of datasets, either through commissioning original content or developing advanced detection software for synthetic data . However, these systems face significant drawbacks, such as the potential lack of diversity in the content and mode collapse. The challenge of aligning profit motives with the ethical use and quality of data raises further concerns (\href{https://time.com/6247678/openai-chatgpt-kenya-workers/}{Time}).

% Conversely, Open GenAI systems allow for a wider array of contributors, potentially fostering greater diversity in training data and resulting outputs. Decentralized models in such ecosystems could lead to more rapid adaptation and diversification of generative models. However, these open systems may also struggle with maintaining consistent quality standards across diverse and extensive datasets. Addressing data privacy and consent may be complex in such decentralized settings. 



% \paragraph{Hardware and efficiency improvements and environmental impacts}

% \paragraph{Crime and malicous use}

==> sections/6_long_term/6_long_term.tex <==
\section{Long-term Impact of Open Source Models}
